Salute the Classic: Revisiting Challenges of Machine Translation in the Age of Large Language Models

The evolution of Neural Machine Translation (NMT) has been significantly influenced by six core challenges (Koehn and Knowles, 2017), which have acted as benchmarks for progress in this field. This study revisits these challenges, offering insights into their ongoing relevance in the context of advanced Large Language Models (LLMs): domain mismatch, amount of parallel data, rare word prediction, translation of long sentences, attention model as word alignment, and sub-optimal beam search. Our empirical findings indicate that LLMs effectively lessen the reliance on parallel data for major languages in the pretraining phase. Additionally, the LLM-based translation system significantly enhances the translation of long sentences that contain approximately 80 words and shows the capability to translate documents of up to 512 words. However, despite these significant improvements, the challenges of domain mismatch and prediction of rare words persist. While the challenges of word alignment and beam search, specifically associated with NMT, may not apply to LLMs, we identify three new challenges for LLMs in translation tasks: inference efficiency, translation of low-resource languages in the pretraining phase, and human-aligned evaluation. The datasets and models are released at https://github.com/pangjh3/LLM4MT.

==> sections/c1_domain_mismatch_13B.tex <==
\subsubsection{Scaling Up to Llama2-13B}



==> sections/new_experiments.tex <==
\section{Add}

==> tablesandfigures/bk/c3_bk2.tex <==
% \pgfplotsset{compat=1.17}

\begin{figure*}
    \centering

% \begin{tikzpicture}
%   \begin{axis}[
%     height=2.3in,
%     width=0.9\textwidth,
%     xmin=0, xmax=500,
%     ymin=0, ymax=100,
%     ybar interval,
%     xtick={0,113,209,271,353,492,657,840,1084,1379,1759,2184,2738,3347,4027,6685},
%     xticklabels={
%       0,4,32,64,128,256,512,999,
%       1999,3999,7999,15999,31999,63999,64000+
%     },
%     x tick label style={rotate=90, anchor=east, font=\small},
%     ymin=0,
%     ymax=100,
%     ytick={0,10,...,100},
%     extra x ticks={80,102,141,163},
%     extra x tick labels={1,2,8,16},
%     extra x tick style={
%       grid=major
%     },
%     ]
%     \addplot coordinates {
%       (0,50.65)
%       (80,52.05)
%       (102,20.51)
%       (113,34.55)
%       (141,44.47)
%       (163,52.06)
%       (209,50.61)
%       (271,58.07)
%       (353,60.38)
%       (492,60.20)
%       (657,69.25)
%       (840,68.51)
%       (1084,69.36)
%       (1379,74.44)
%       (1759,80.34)
%       (2184,80.65)
%       (2738,80.17)
%       (3347,81.73)
%       (4027,81.93)
%       (6685,0)
%     };
%     % \node at (axis cs:102,-5) [anchor=north,rotate=90] {1};
%     % \node at (axis cs:113,-10) [anchor=north,rotate=90] {2};
%     % \node at (axis cs:141,-15) [anchor=north,rotate=90] {8};
%     % \node at (axis cs:163,-20) [anchor=north,rotate=90] {16};
%   \end{axis}
% \end{tikzpicture}

\begin{tikzpicture}
  \begin{axis}[
    height=2.3in,
    width=1.0\textwidth,
    xmin=0, xmax=6685,
    ymin=0, ymax=100,
    ybar interval,
    xtick={0,113,209,271,353,492,657,840,1084,1379,1759,2184,2738,3347,4027,6685},
    xticklabels={
      0, 4, 32, 64, 128, 256, 512, 999,
      1999, 3999, 7999, 15999, 31999, 63999, 64000+
    },
    x tick label style={rotate=90, anchor=east, font=\small},
    y tick label style={font=\small},
    ymin=0,
    ymax=100,
    ytick={0,10,...,100},
    grid=none
    ]
    \addplot [fill=lightblue, draw=none] coordinates {
      (0,50.65)
      (80,52.05)
      (102,20.51)
      (113,34.55)
      (141,44.47)
      (163,52.06)
      (209,50.61)
      (271,58.07)
      (353,60.38)
      (492,60.20)
      (657,69.25)
      (840,68.51)
      (1084,69.36)
      (1379,74.44)
      (1759,80.34)
      (2184,80.65)
      (2738,80.17)
      (3347,81.73)
      (4027,81.93)
      (6685,0)
    };
    \draw (axis cs:91,12) -- (axis cs:-200,8) node[below, anchor=center, rotate=30,pos=1.2] {1};
    \draw (axis cs:107.5,12) -- (axis cs:-50,5) node[below] {2};
    \draw (axis cs:136,12) -- (axis cs:141,2) node[below] {8};
    \draw (axis cs:152,12) -- (axis cs:400,0) node[below] {16};
  \end{axis}

\begin{axis}[
    height=2.3in,
    width=1.0\textwidth,
    xmin=0, xmax=6685,
    ymin=0, ymax=100,
    ybar interval,
    xtick={0,113,209,271,353,492,657,840,1084,1379,1759,2184,2738,3347,4027,6685},
    xticklabels={
      0, 4, 32, 64, 128, 256, 512, 999,
      1999, 3999, 7999, 15999, 31999, 63999, 64000+
    },
    x tick label style={rotate=90, anchor=east, font=\small},
    y tick label style={font=\small},
    ymin=0,
    ymax=100,
    ytick={0,10,...,100},
    grid=none
    ]
    \addplot [fill=darkgreen, draw=none,] coordinates {
      (0,50.82)
      (80,50.86)
      (102,25.00)
      (113,38.55)
      (141,46.89)
      (163,54.34)
      (209,47.55)
      (271,51.38)
      (353,57.73)
      (492,54.88)
      (657,60.46)
      (840,63.71)
      (1084,64.88)
      (1379,70.78)
      (1759,75.14)
      (2184,73.27)
      (2738,75.35)
      (3347,75.13)
      (4027,73.95)
      (6685,0)
    };
    \node at (axis cs:102,-5) [anchor=north,rotate=90] {1};
    \node at (axis cs:113,-10) [anchor=north,rotate=90] {2};
    \node at (axis cs:141,-15) [anchor=north,rotate=90] {8};
    \node at (axis cs:163,-20) [anchor=north,rotate=90] {16};

  \end{axis}

\begin{axis}[
    height=2.3in,
    width=1.0\textwidth,
    xmin=0, xmax=6685,
    ymin=0, ymax=100,
    ybar interval,
    xtick={0,113,209,271,353,492,657,840,1084,1379,1759,2184,2738,3347,4027,6685},
    xticklabels={
      0, 4, 32, 64, 128, 256, 512, 999,
      1999, 3999, 7999, 15999, 31999, 63999, 64000+
    },
    x tick label style={rotate=90, anchor=east, font=\small},
    y tick label style={font=\small},
    ymin=0,
    ymax=100,
    ytick={0,10,...,100},
    grid=none
    ]
    \addplot [fill=lightgray, draw=none] coordinates {
      (0,50.65)
      (80,52.05)
      (102,20.51)
      (113,34.55)
      (141,44.47)
      (163,52.06)
      (209,47.55)
      (271,51.38)
      (353,57.73)
      (492,54.88)
      (657,60.46)
      (840,63.71)
      (1084,64.88)
      (1379,70.78)
      (1759,75.14)
      (2184,73.27)
      (2738,75.35)
      (3347,75.13)
      (4027,73.95)
      (6685,0)
    };

  \end{axis}



\end{tikzpicture}


    \caption{Caption}
    \label{fig:rarewords}
\end{figure*}




==> tablesandfigures/bk/c3_goodbk.tex <==
% \pgfplotsset{compat=1.17}

\begin{figure*}
    \centering

\begin{tikzpicture}
\useasboundingbox (3.5cm,-2cm) rectangle (10cm,3.5cm);

  \begin{axis}[
    height=2in,
    width=1.0\textwidth,
    xmin=0, xmax=6685,
    ymin=15, ymax=85,
    ybar interval,
    xtick={0,113,209,271,353,492,657,840,1084,1379,1759,2184,2738,3347,4027,6685},
    xticklabels={
      0, 4, 32, 64, 128, 256, 512, 999,
      1999, 3999, 7999, 15999, 31999, 63999, 64000+
    },
    x tick label style={rotate=90, anchor=east, font=\small},
    y tick label style={font=\small},
    ytick={15,25,35,45,55,65,75},
    yticklabels={15\%,25\%,35\%,45\%,55\%,65\%,75\%},
    grid=none,
    axis lines=left,
    x axis line style={opacity=0},
    y axis line style={opacity=0},
    tick style={draw=none},
    clip mode=individual,
    ]
    \addplot[fill=lightblue, draw=none,draw=white,line width=0.1pt] coordinates {
      (0,50.65)
      (80,52.05)
      (102,20.51)
      (113,34.55)
      (141,44.47)
      (163,52.06)
      (209,50.61)
      (271,58.07)
      (353,60.38)
      (492,60.20)
      (657,69.25)
      (840,68.51)
      (1084,69.36)
      (1379,74.44)
      (1759,80.34)
      (2184,80.65)
      (2738,80.17)
      (3347,81.73)
      (4027,81.93)
      (6685,0)
    };

        \draw (axis cs:91,12) -- (axis cs:-200,8) node[below, anchor=center, rotate=30,pos=1.2,font=\small] {1};
    \draw (axis cs:107.5,12) -- (axis cs:-50,5) node[below, anchor=center, rotate=40,pos=1.2,font=\small] {2};
    \draw (axis cs:136,12) -- (axis cs:141,2) node[below, anchor=center, rotate=91,pos=1.2,font=\small] {8};
    \draw (axis cs:152,12) -- (axis cs:350,0) node[below, anchor=center, rotate=120,pos=1.3,font=\small] {16};
\end{axis}


\begin{axis}[
    height=2in,
    width=1.0\textwidth,
    xmin=0, xmax=6685,
    ymin=15, ymax=85,
    ybar interval,
    xtick={0,113,209,271,353,492,657,840,1084,1379,1759,2184,2738,3347,4027,6685},
    xticklabels={
      0, 4, 32, 64, 128, 256, 512, 999,
      1999, 3999, 7999, 15999, 31999, 63999, 64000+
    },
    x tick label style={rotate=90, anchor=east, font=\small},
    y tick label style={font=\small},
    ytick={15,25,35,45,55,65,75},
    yticklabels={15\%,25\%,35\%,45\%,55\%,65\%,75\%},
    grid=none,
    axis lines=left,
    x axis line style={opacity=0},
    y axis line style={opacity=0},
    tick style={draw=none},
    ]
    \addplot[fill=darkgreen, draw=none,draw=white,line width=0.1pt] coordinates {
      (0,50.82)
      (80,50.86)
      (102,25.00)
      (113,38.55)
      (141,46.89)
      (163,54.34)
      (209,47.55)
      (271,51.38)
      (353,57.73)
      (492,54.88)
      (657,60.46)
      (840,63.71)
      (1084,64.88)
      (1379,70.78)
      (1759,75.14)
      (2184,73.27)
      (2738,75.35)
      (3347,75.13)
      (4027,73.95)
      (6685,0)
    };
\end{axis}


\begin{axis}[
    height=2in,
    width=1.0\textwidth,
    xmin=0, xmax=6685,
    ymin=15, ymax=85,
    ybar interval,
    xtick={0,113,209,271,353,492,657,840,1084,1379,1759,2184,2738,3347,4027,6685},
    xticklabels={
      0, 4, 32, 64, 128, 256, 512, 999,
      1999, 3999, 7999, 15999, 31999, 63999, 64000+
    },
    x tick label style={rotate=90, anchor=east, font=\small},
    y tick label style={font=\small},
    ytick={15,25,35,45,55,65,75},
    yticklabels={15\%,25\%,35\%,45\%,55\%,65\%,75\%},
    grid=none,
    axis lines=left,
    x axis line style={opacity=0},
    y axis line style={opacity=0},
    tick style={draw=none},
    ]
    \addplot[fill=overlapcl, draw=white,line width=0.1pt] coordinates {
 (0.00,50.65)
(80,50.86)
(102,20.51)
(113,34.55)
(141,44.47)
(163,52.06)
(209,47.55)
(271,51.38)
(353,57.73)
(492,54.88)
(657,60.46)
(840,63.71)
(1084,64.88)
(1379,70.78)
(1759,75.14)
(2184,73.27)
(2738,75.35)
(3347,75.13)
(4027,73.95)
(6685,0)
    };

\begin{pgfonlayer}{foreground}
\addplot[const plot, no markers,color=blue,line width=2pt] coordinates {
      (0,50.65)
      (80,52.05)
      (102,20.51)
      (113,34.55)
      (141,44.47)
      (163,52.06)
      (209,50.61)
      (271,58.07)
      (353,60.38)
      (492,60.20)
      (657,69.25)
      (840,68.51)
      (1084,69.36)
      (1379,74.44)
      (1759,80.34)
      (2184,80.65)
      (2738,80.17)
      (3347,81.73)
      (4027,81.93)
      (6685,81.93)
    };
\addplot[const plot, no markers,color=forestgreen,line width=2pt] coordinates {
      (0,50.82)
      (80,50.86)
      (102,25.00)
      (113,38.55)
      (141,46.89)
      (163,54.34)
      (209,47.55)
      (271,51.38)
      (353,57.73)
      (492,54.88)
      (657,60.46)
      (840,63.71)
      (1084,64.88)
      (1379,70.78)
      (1759,75.14)
      (2184,73.27)
      (2738,75.35)
      (3347,75.13)
      (4027,73.95)
      (6685,73.95)
    };
\end{pgfonlayer}
    
\end{axis}


\begin{axis}[
    height=5cm,
    width=1.0\textwidth,
    xmin=0, xmax=6685,
    ymin=-85, ymax=0,
    ybar interval,
    xtick={0,113,209,271,353,492,657,840,1084,1379,1759,2184,2738,3347,4027,6685},
    xticklabels={
      0, 4, 32, 64, 128, 256, 512, 999,
      1999, 3999, 7999, 15999, 31999, 63999, 64000+
    },
    x tick label style={rotate=90, anchor=east, font=\small,opacity=0},
    y tick label style={font=\small},
    ytick={-10,0},
    yticklabels={10\%,0\%},
    grid=none,
    axis lines=left,
    x axis line style={opacity=0},
    y axis line style={opacity=0},
    yshift=-4.8cm,
    tick style={draw=none},
    ]
    \addplot[fill=lightblue, draw=white,line width=0.1pt] coordinates {
    (0,-6.567504677)
    (80,-3.846153846)
    (102,0)
    (113,-13.46153846)
    (141,-8.695652174)
    (163,-6.25)
    (209,-6.756756757)
    (271,-3.977272727)
    (353,-6)
    (492,-8.196721311)
    (657,-6.220095694)
    (840,-5.620155039)
    (1084,-6.401515152)
    (1379,-4.830917874)
    (1759,-3.563544623)
    (2184,-4.908306365)
    (2738,-4.878909442)
    (3347,-3.966088482)
    (4027,-4.591777536)
    (6685,0)
};

\end{axis}

\begin{axis}[
    height=5cm,
    width=1.0\textwidth,
    xmin=0, xmax=6685,
    ymin=-85, ymax=0,
    ybar interval,
    xtick={0,113,209,271,353,492,657,840,1084,1379,1759,2184,2738,3347,4027,6685},
    xticklabels={
      0, 4, 32, 64, 128, 256, 512, 999,
      1999, 3999, 7999, 15999, 31999, 63999, 64000+
    },
    x tick label style={rotate=90, anchor=east, font=\small,opacity=0},
    y tick label style={font=\small},
    ytick={-10,0},
    yticklabels={10\%,0\%},
    grid=none,
    axis lines=left,
    x axis line style={opacity=0},
    y axis line style={opacity=0},
    yshift=-4.8cm,
    tick style={draw=none},
    ]
    \addplot[fill=darkgreen, draw=white,line width=0.1pt] coordinates {
(0,-8.24742268)
(80,-14)
(102,0)
(113,-8.695652174)
(141,-9.090909091)
(163,-4.444444444)
(209,-16.85714286)
(271,-18.27586207)
(353,-10.81050228)
(492,-14.65517241)
(657,-14.15410385)
(840,-12.4831309)
(1084,-10.38049303)
(1379,-10.12507535)
(1759,-8.796934866)
(2184,-9.795221843)
(2738,-11.98281949)
(3347,-10.65732023)
(4027,-12.08899534)
(6685,0)
};
\end{axis}

\begin{axis}[
    height=5cm,
    width=1.0\textwidth,
    xmin=0, xmax=6685,
    ymin=-85, ymax=0,
    ybar interval,
    xtick={0,113,209,271,353,492,657,840,1084,1379,1759,2184,2738,3347,4027,6685},
    xticklabels={
      0, 4, 32, 64, 128, 256, 512, 999,
      1999, 3999, 7999, 15999, 31999, 63999, 64000+
    },
    x tick label style={rotate=90, anchor=east, font=\small,opacity=0},
    y tick label style={font=\small},
    ytick={-10,0},
    yticklabels={10\%,0\%},
    grid=none,
    axis lines=left,
    x axis line style={opacity=0},
    y axis line style={opacity=0},
    yshift=-4.8cm,
    tick style={draw=none},
    ]
    \addplot[fill=overlapcl, draw=white,line width=0.1pt] coordinates {
(0,-6.567504677)
(80,-3.846153846)
(102,0)
(113,-8.695652174)
(141,-8.695652174)
(163,-4.444444444)
(209,-6.756756757)
(271,-3.977272727)
(353,-6)
(492,-8.196721311)
(657,-6.220095694)
(840,-5.620155039)
(1084,-6.401515152)
(1379,-4.830917874)
(1759,-3.563544623)
(2184,-4.908306365)
(2738,-4.878909442)
(3347,-3.966088482)
(4027,-4.591777536)
(6685,0)
    };

\begin{pgfonlayer}{foreground}
\addplot[const plot, no markers,color=blue,line width=2pt] coordinates {
    (0,-6.567504677)
    (80,-3.846153846)
    (102,0)
    (113,-13.46153846)
    (141,-8.695652174)
    (163,-6.25)
    (209,-6.756756757)
    (271,-3.977272727)
    (353,-6)
    (492,-8.196721311)
    (657,-6.220095694)
    (840,-5.620155039)
    (1084,-6.401515152)
    (1379,-4.830917874)
    (1759,-3.563544623)
    (2184,-4.908306365)
    (2738,-4.878909442)
    (3347,-3.966088482)
    (4027,-4.591777536)
    (6685,-4.591777536)
    };
    
\addplot[const plot, no markers,color=forestgreen,line width=2pt] coordinates {
(0,-8.24742268)
(80,-14)
(102,0)
(113,-8.695652174)
(141,-9.090909091)
(163,-4.444444444)
(209,-16.85714286)
(271,-18.27586207)
(353,-10.81050228)
(492,-14.65517241)
(657,-14.15410385)
(840,-12.4831309)
(1084,-10.38049303)
(1379,-10.12507535)
(1759,-8.796934866)
(2184,-9.795221843)
(2738,-11.98281949)
(3347,-10.65732023)
(4027,-12.08899534)
(6685,-12.08899534)
    };
\end{pgfonlayer}
    
\end{axis}



\end{tikzpicture}


    \caption{Precision of translation and delete rates by source word frequency. The \textcolor{lightblue}{light blue} and \textcolor{darkgreen}{ dark green} indicate the LLM and Enc2Dec translation models. The horizontal axis represents the frequency of source word types in the test corpus, where axis labels indicate the upper limit of each frequency range, and the bin width is proportional to the number of word types in that range. The precision and deletion rates are shown on the upper and lower vertical axes respectively. LLMs excel at predicting words that appear more than eight times but perform poorly with rare words. The detail information are listed in Table~\ref{tab:app_c3}.}
    \label{fig:rarewords}
\end{figure*}








==> tablesandfigures/c1_md_bleu_and_examples.tex <==
\begin{table*}[h]
  \centering
  \small
  \begin{subtable}[h]{1.0\textwidth}
  \scalebox{0.8}{
  \begin{tabular}{l|c|c|c|c|c}
    \toprule
    System$\downarrow$ & Law & Medical & IT & Koran & Subtitles \\ \midrule \midrule
    \multirow{-1.6}{*}{All Data}
    % & \DrawPercentageBar{57.2}{61.5}
    % & \DrawPercentageBar{53.3}{59.7}
    % & \DrawPercentageBar{42.1}{47.5}
    % & \DrawPercentageBar{20.9}{18.6}
    % & \DrawPercentageBar{27.6}{27.0} \\ \midrule
    & \DrawPercentageBar{56.4}{61.5}
    & \DrawPercentageBar{51.4}{59.7}
    & \DrawPercentageBar{41.7}{47.5}
    & \DrawPercentageBar{20.1}{18.6}
    & \DrawPercentageBar{26.8}{27.0} \\ \midrule
    

    \multirow{-1.6}{*}{Law}
    & \DrawPercentageBar{59.0}{62.0}
    & \DrawPercentageBar{21.7}{36.1}
    & \DrawPercentageBar{13.1}{29.6}
    & \DrawPercentageBar{2.7}{12.0}
    & \DrawPercentageBar{5.4}{20.4} \\ \midrule

    \multirow{-1.6}{*}{Medical}
    & \DrawPercentageBar{18.3}{28.52}
    & \DrawPercentageBar{56.5}{59.31}
    & \DrawPercentageBar{11.4}{31.2}
    & \DrawPercentageBar{1.9}{11.8}
    & \DrawPercentageBar{4.3}{19.9} \\ \midrule


    \multirow{-1.6}{*}{IT}
    & \DrawPercentageBar{9.6}{30.3}
    & \DrawPercentageBar{14.9}{36.9}
    & \DrawPercentageBar{43.0}{47.4}
    & \DrawPercentageBar{2.8}{11.7}
    & \DrawPercentageBar{8.6}{23.1} \\ \midrule

    \multirow{-1.6}{*}{Koran}
    & \DrawPercentageBar{0.2}{22.3}
    & \DrawPercentageBar{0.1}{28.15}
    & \DrawPercentageBar{0.2}{16.8}
    & \DrawPercentageBar{15.9}{20.3}
    & \DrawPercentageBar{0.5}{10.6} \\ \midrule

    \multirow{-1.6}{*}{Subtitles}
    & \DrawPercentageBar{5.5}{27.13}
    & \DrawPercentageBar{7.9}{33.5}
    & \DrawPercentageBar{8.5}{26.9}
    & \DrawPercentageBar{6.4}{11.6}
    & \DrawPercentageBar{27.3}{28.1}


    \\ \bottomrule
  \end{tabular}
  }
  \caption{Translation quality (BLEU scores) of multi-domain tasks, where the system is trained on one domain (rows) and tested on another domain (columns).}
  \label{tab:c1_multi_domain}
\end{subtable}

\begin{subtable}[h]{1.0\textwidth}

    \scalebox{0.9}{
    \begin{tabular}{l|p{4.5cm}|p{4.5cm}|p{4.5cm}} 
    \toprule
         &  1: Medical & 2: IT & 3: Subtitles \\ \midrule
      Source  &  The pipettes must be kept in sterile packaging. & Methode fÃ¼r die Berechnung der Vorhersage & Du kannst ihr nicht helfen, außer dass du jetzt den Tatort untersuchst. \\ \midrule
      Ref. & Stored pipettes must be kept in the intact foil package. & Method to calculate forecast & You can't do anything but help her by working the crime scene. \\ \midrule
      \midrule
      All & Pipettes must be stored in the intact foil pouch. & Method to calculate the forecast & You can't help her except by \textcolor{red}{canvassing the scene}. \\ \midrule
      Law & The pipettes must be stored in the intact \textcolor{red}{sheet} pack. & Method \textcolor{red}{of calculation} of the forecast
 & You can't help her, except by \textcolor{red}{examining the scene of the crime}. \\ \midrule
      Medical & The pipettes must be stored in the intact foil pouch. &  \textcolor{red}{Prediction method}
 & You can’ t help her now, except by \textcolor{red}{examining the scene of the accident}. \\ \midrule
      IT & The pipettes must be stored in the intact \textcolor{red}{slide} pack. & Method \textcolor{red}{for calculating} the forecast
  & You can't help her, except by \textcolor{red}{examining the crime scene}. \\ \midrule
      Koran & The pipettes must be kept in \textcolor{red}{sterile} packaging. & \textcolor{red}{A method} to calculate the prediction.
 & \textcolor{red}{If you do not}, you will not be able to help her. \\ \midrule
      Subtitles & The pipettes must be stored in intact \textcolor{red}{slide wraps}. &  Method \textcolor{red}{for calculating} the forecast
 & You can't help her, except to process the crime scene.  \\ \bottomrule
    \end{tabular}
    }
    \caption{Test examples from three domains, which are translated by the translation trained on the domain in the first column. We use red color to tag the translation mismatch in the hypothesis.}
    \label{tab:mdexamples}

\end{subtable}
  
\end{table*}





==> tablesandfigures/c1_md_with13B.tex <==
\begin{table*}[ht]
\small
  \centering
\resizebox{\textwidth}{!}{
  \begin{tabular}{lccccc}
    \toprule
    \bf System$\downarrow$ & \bf Law & \bf Medical & \bf IT & \bf Koran & \bf Subtitles \\ \midrule
    \multirow{-1.6}{*}{\bf All Data}
    % & \DrawPercentageBar{57.2}{61.5}
    % & \DrawPercentageBar{53.3}{59.7}
    % & \DrawPercentageBar{42.1}{47.5}
    % & \DrawPercentageBar{20.9}{18.6}
    % & \DrawPercentageBar{27.6}{27.0} \\ \midrule
    & \DrawThreePercentageBar{64.3}{61.5}{56.4}
    & \DrawThreePercentageBar{61.5}{59.7}{51.4}
    & \DrawThreePercentageBar{50.6}{47.5}{41.7}
    & \DrawThreePercentageBar{20.3}{18.6}{20.1}
    & \DrawThreePercentageBar{28.8}{27.0}{26.8} \\ \midrule
    

    \multirow{-1.6}{*}{\bf Law}
    & \cellcolor[rgb]{0.85,0.85,0.85}\DrawThreePercentageBar{63.9}{62.0}{59.0}
    & \DrawThreePercentageBar{38.3}{36.1}{21.7}
    & \DrawThreePercentageBar{31.1}{29.6}{13.1}
    & \DrawThreePercentageBar{14.5}{12.0}{2.7}
    & \DrawThreePercentageBar{22.3}{20.4}{5.4} \\ \midrule

    \multirow{-1.6}{*}{\bf Medical}
    & \DrawThreePercentageBar{30.2}{28.5}{18.3}
    & \cellcolor[rgb]{0.85,0.85,0.85}\DrawThreePercentageBar{61.4}{59.31}{56.5}
    & \DrawThreePercentageBar{29.2}{31.2}{11.4}
    & \DrawThreePercentageBar{13.6}{11.8}{1.9}
    & \DrawThreePercentageBar{22.0}{19.9}{4.3} \\ \midrule


    \multirow{-1.6}{*}{\bf IT}
    & \DrawThreePercentageBar{32.8}{30.3}{9.6}
    & \DrawThreePercentageBar{38.5}{36.9}{14.9}
    & \cellcolor[rgb]{0.85,0.85,0.85}\DrawThreePercentageBar{51.0}{47.4}{43.0}
    & \DrawThreePercentageBar{14.4}{11.7}{2.8}
    & \DrawThreePercentageBar{24.2}{23.1}{8.6} \\ \midrule

    \multirow{-1.6}{*}{\bf Koran}
    & \DrawThreePercentageBar{23.1}{22.3}{0.2}
    & \DrawThreePercentageBar{27.5}{28.15}{0.1}
    & \DrawThreePercentageBar{19.2}{16.8}{0.2}
    & \cellcolor[rgb]{0.85,0.85,0.85}\DrawThreePercentageBar{20.6}{20.3}{15.9}
    & \DrawThreePercentageBar{10.8}{10.6}{0.5} \\ \midrule

    \multirow{-1.6}{*}{\bf Subtitles}
    & \DrawThreePercentageBar{28.9}{27.1}{5.5}
    & \DrawThreePercentageBar{33.4}{33.5}{7.9}
    & \DrawThreePercentageBar{26.7}{26.9}{8.5}
    & \DrawThreePercentageBar{13.2}{11.6}{6.4}
    & \cellcolor[rgb]{0.85,0.85,0.85}\DrawThreePercentageBar{28.9}{28.1}{27.3}


    \\ \bottomrule
  \end{tabular}
  }
  \caption{\textcolor{red}{Translation quality (BLEU scores) of multi-domain German-to-English translation tasks, where the system is trained on one domain (rows) and tested on another domain (columns). The {\color{black}black}, {\color{red}red}, and {\color{blue}blue} bars refer to the LLM-SFT-13B, LLM-SFT, and Enc2Dec models, respectively. LLMs improve the in-domain and out-of-domain translation qualities but still suffer from the domain mismatch problem.}}
  
  \label{tab:c1_multi_domain}
\end{table*}





==> tablesandfigures/c1_multi_domain.tex <==
\begin{table*}[ht]
\small
  \centering
  \scalebox{0.95}{
  \begin{tabular}{lccccc}
    \toprule
    \bf System$\downarrow$ & \bf Law & \bf Medical & \bf IT & \bf Koran & \bf Subtitles \\ \midrule
    \multirow{-1.6}{*}{\bf All Data}
    % & \DrawPercentageBar{57.2}{61.5}
    % & \DrawPercentageBar{53.3}{59.7}
    % & \DrawPercentageBar{42.1}{47.5}
    % & \DrawPercentageBar{20.9}{18.6}
    % & \DrawPercentageBar{27.6}{27.0} \\ \midrule
    & \DrawPercentageBar{61.5}{56.4}
    & \DrawPercentageBar{59.7}{51.4}
    & \DrawPercentageBar{47.5}{41.7}
    & \DrawPercentageBar{18.6}{20.1}
    & \DrawPercentageBar{27.0}{26.8} \\ \midrule
    

    \multirow{-1.6}{*}{\bf Law}
    & \cellcolor[rgb]{0.85,0.85,0.85}\DrawPercentageBar{62.0}{59.0}
    & \DrawPercentageBar{36.1}{21.7}
    & \DrawPercentageBar{29.6}{13.1}
    & \DrawPercentageBar{12.0}{2.7}
    & \DrawPercentageBar{20.4}{5.4} \\ \midrule

    \multirow{-1.6}{*}{\bf Medical}
    & \DrawPercentageBar{28.5}{18.3}
    & \cellcolor[rgb]{0.85,0.85,0.85}\DrawPercentageBar{59.31}{56.5}
    & \DrawPercentageBar{31.2}{11.4}
    & \DrawPercentageBar{11.8}{1.9}
    & \DrawPercentageBar{19.9}{4.3} \\ \midrule


    \multirow{-1.6}{*}{\bf IT}
    & \DrawPercentageBar{30.3}{9.6}
    & \DrawPercentageBar{36.9}{14.9}
    & \cellcolor[rgb]{0.85,0.85,0.85}\DrawPercentageBar{47.4}{43.0}
    & \DrawPercentageBar{11.7}{2.8}
    & \DrawPercentageBar{23.1}{8.6} \\ \midrule

    \multirow{-1.6}{*}{\bf Koran}
    & \DrawPercentageBar{22.3}{0.2}
    & \DrawPercentageBar{28.15}{0.1}
    & \DrawPercentageBar{16.8}{0.2}
    & \cellcolor[rgb]{0.85,0.85,0.85}\DrawPercentageBar{20.3}{15.9}
    & \DrawPercentageBar{10.6}{0.5} \\ \midrule

    \multirow{-1.6}{*}{\bf Subtitles}
    & \DrawPercentageBar{27.1}{5.5}
    & \DrawPercentageBar{33.5}{7.9}
    & \DrawPercentageBar{26.9}{8.5}
    & \DrawPercentageBar{11.6}{6.4}
    & \cellcolor[rgb]{0.85,0.85,0.85}\DrawPercentageBar{28.1}{27.3}


    \\ \bottomrule
  \end{tabular}
  }
  \caption{Translation quality (BLEU scores) of multi-domain German-to-English translation tasks, where the system is trained on one domain (rows) and tested on another domain (columns). The {\color{red}red} and {\color{blue}blue} bars refer to the LLM and Enc2Dec models, respectively. LLMs improve the in-domain and out-of-domain translation qualities but still suffer from the domain mismatch problem.}
  % \caption{Translation quality (BLEU scores) of multi-domain tasks, where the system is trained on one domain (rows) and tested on another domain (columns). The red and blue bars refer to the LLM and Enc2Dec models, respectively.}
  
  \label{tab:c1_multi_domain}
\end{table*}




% \begin{table*}[h]
%   \centering
%   \begin{tabular}{c|c|c|c|c|c}
%     \toprule
%     System$\downarrow$ & Law & Medical & IT & Koran & Subtitles \\ \midrule \midrule
%     All Data
%     & 
%     \begin{minipage}{0.3\columnwidth}
% 	\centering
% 	$\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$
%     \end{minipage}
%     & 
%     \begin{minipage}{0.3\columnwidth}
% 	\centering
% 	$\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$
%     \end{minipage}
%     & 
%     \begin{minipage}{0.3\columnwidth}
% 	\centering
% 	$\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$
%     \end{minipage}
%     & 
%     \begin{minipage}{0.3\columnwidth}
% 	\centering
% 	$\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$
%     \end{minipage}
%     & 
%     \begin{minipage}{0.3\columnwidth}
% 	\centering
% 	$\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$
%     \end{minipage}  \\ \midrule

%     Law
%     & 
%     \begin{minipage}{0.3\columnwidth}
% 	\centering
% 	$\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$
%     \end{minipage}
%     & 
%     \begin{minipage}{0.3\columnwidth}
% 	\centering
% 	$\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$
%     \end{minipage}
%     & 
%     \begin{minipage}{0.3\columnwidth}
% 	\centering
% 	$\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$
%     \end{minipage}
%     & 
%     \begin{minipage}{0.3\columnwidth}
% 	\centering
% 	$\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$
%     \end{minipage}
%     & 
%     \begin{minipage}{0.3\columnwidth}
% 	\centering
% 	$\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$
%     \end{minipage} 

%     \\ \bottomrule
%   \end{tabular}
%   \caption{Name of this table}
% \end{table*}


% \begin{table*}[h]
%   \centering
%   \begin{tabular}{c|c|c|c|c|c}
%     \toprule
%     Items & Advantages & Disadvantages \\ \midrule
%     All Data
%     & 
%     $\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$
%     & 
%     $\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$
%     & 
%     $\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$
%     & 
%     $\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$
%     & 
%     $\raisebox{-.5\height}{\input{tablesandfigures/c2_result_figures/law2law}}$

%     \\ \bottomrule
%   \end{tabular}
%   \caption{Name of this table}
% \end{table*}


==> tablesandfigures/c3_rare_word_apptable.tex <==
% \begin{table*}[ht]
% \centering
% \begin{tabular}{llcccc}
% \toprule
%  \multirow{2}{*}{\bf Freq. Upper Bounds}    & \multirow{2}{*}{\bf Word Type Count}    & \multicolumn{2}{c}{\bf LLM-SFT} & \multicolumn{2}{c}{\bf Enc2Dec} \\ \cmidrule{3-4} \cmidrule{5-6} 
%  &  & \bf ACC (\%)         &  \bf Delete (\%)       & \bf ACC (\%)          & \bf Delete (\%)         \\ \midrule
% 0                    & 80              & 50.65        & 6.57         & 50.82        & 8.25         \\
% 1                    & 22              & 52.05        & 3.85         & 50.86        & 14.00        \\
% 2                    & 11              & 20.51        & 0.00         & 25.00        & 0.00         \\
% 4                    & 28              & 34.55        & 13.46        & 38.55        & 8.70         \\
% 8                    & 22              & 44.47        & 8.70         & 46.89        & 9.09         \\
% 16                   & 46              & 52.06        & 6.25         & 54.34        & 4.44         \\
% 32                   & 62              & 50.61        & 6.76         & 47.55        & 16.86        \\
% 64                   & 82              & 58.07        & 3.98         & 51.38        & 18.28        \\
% 128                  & 139             & 60.38        & 6.00         & 57.73        & 10.81        \\
% 256                  & 165             & 60.20        & 8.20         & 54.88        & 14.66        \\
% 512                  & 183             & 69.25        & 6.22         & 60.46        & 14.15        \\
% 999                  & 244             & 68.51        & 5.62         & 63.71        & 12.48        \\
% 1999                 & 295             & 69.36        & 6.40         & 64.88        & 10.38        \\
% 3999                 & 380             & 74.44        & 4.83         & 70.78        & 10.13        \\
% 7999                 & 425             & 80.34        & 3.56         & 75.14        & 8.80         \\
% 15999                & 554             & 80.65        & 4.91         & 73.27        & 9.80         \\
% 31999                & 609             & 80.17        & 4.88         & 75.35        & 11.98        \\
% 63999                & 680             & 81.73        & 3.97         & 75.13        & 10.66        \\
% 64000+               & 2658            & 81.93        & 4.59         & 73.95        & 12.09 \\ \cdashline{1-6}\noalign{\vskip 0.5ex}
% Average & 352  & 61.58 & 5.72 & 58.46 & 10.82 \\ 

% \bottomrule
% \end{tabular}
% \caption{Precision of translation and delete rates for source word types of frequency.}
% \label{tab:apprareword}
% \end{table*}


% \begin{table*}[ht]
% \centering
% \begin{tabular}{llcccccc}
% \toprule
%   \multirow{2}{*}{\bf Freq. Bin}    & \multirow{2}{*}{\bf Counts}         & \multicolumn{2}{c}{\bf LLM-SFT} & \multicolumn{2}{c}{\bf LLM-SFT-S0.7} & \multicolumn{2}{c}{\bf Enc2Dec} \\ \cmidrule{3-4} \cmidrule{5-6} \cmidrule{7-8}
%  & & \bf ACC(\%)          &  \bf Delete(\%)         & \bf ACC(\%)              &  \bf Delete(\%)            & 
%  \bf ACC(\%)            & \bf Delete(\%)        \\ \midrule
% 0                    & 80              & 50.65        & 6.57         & 53.55          & 3.54            & 50.82        & 8.25         \\
% 1                    & 22              & 52.05        & 3.85         & 61.08          & 3.85            & 50.86        & 14.00        \\
% 2                    & 11              & 20.51        & 0.00         & 21.85          & 0.00            & 25.00        & 0.00         \\
% 4                    & 28              & 34.55        & 13.46        & 33.72          & 13.46           & 38.55        & 8.70         \\
% 8                    & 22              & 44.47        & 8.70         & 37.88          & 13.04           & 46.89        & 9.09         \\
% 16                   & 46              & 52.06        & 6.25         & 54.69          & 0.00            & 54.34        & 4.44         \\
% 32                   & 62              & 50.61        & 6.76         & 51.59          & 13.51           & 47.55        & 16.86        \\
% 64                   & 82              & 58.07        & 3.98         & 57.09          & 6.25            & 51.38        & 18.28        \\
% 128                  & 139             & 60.38        & 6.00         & 56.87          & 10.00           & 57.73        & 10.81        \\
% 256                  & 165             & 60.20        & 8.20         & 64.09          & 5.74            & 54.88        & 14.66        \\
% 512                  & 183             & 69.25        & 6.22         & 66.52          & 8.89            & 60.46        & 14.15        \\
% 999                  & 244             & 68.51        & 5.62         & 64.91          & 9.21            & 63.71        & 12.48        \\
% 1999                 & 295             & 69.36        & 6.40         & 66.65          & 7.69            & 64.88        & 10.38        \\
% 3999                 & 380             & 74.44        & 4.83         & 73.97          & 5.92            & 70.78        & 10.13        \\
% 7999                 & 425             & 80.34        & 3.56         & 77.60          & 6.73            & 75.14        & 8.80         \\
% 15999                & 554             & 80.65        & 4.91         & 77.02          & 7.04            & 73.27        & 9.80         \\
% 31999                & 609             & 80.17        & 4.88         & 78.95          & 6.25            & 75.35        & 11.98        \\
% 63999                & 680             & 81.73        & 3.97         & 78.73          & 5.86            & 75.13        & 10.66        \\
% 64000+               & 2658            & 81.93        & 4.59         & 78.62          & 7.04            & 73.95        & 12.09        \\ \cdashline{1-8}\noalign{\vskip 0.5ex}
% Average                  & 352             & 61.58        & 5.72         & 60.81          & 7.05            & 58.46        & 10.82    \\ \bottomrule
% \end{tabular}
% \caption{Precision of translation and delete rates for source word types of frequency.}
% \label{tab:apprareword}
% \end{table*}


\begin{table*}[ht]
\centering
\begin{tabular}{llcccccc}
\toprule
  \multirow{2}{*}{\bf Freq. Bin}    & \multirow{2}{*}{\bf Counts}         & \multicolumn{2}{c}{\bf LLM-SFT} & \multicolumn{2}{c}{\bf LLM-SFT-S0.1} & \multicolumn{2}{c}{\bf Enc2Dec} \\ \cmidrule{3-4} \cmidrule{5-6} \cmidrule{7-8}
 & & \bf ACC(\%)          &  \bf Delete(\%)         & \bf ACC(\%)              &  \bf Delete(\%)            & 
 \bf ACC(\%)            & \bf Delete(\%)        \\ \midrule
0                    & 80              & 50.65        & 6.57         & 55.79          & 4.12            & 50.82        & 8.25         \\
1                    & 22              & 52.05        & 3.85         & 53.82          & 11.54           & 50.86        & 14.00        \\
2                    & 11              & 20.51        & 0.00         & 21.37          & 0.00            & 25.00        & 0.00         \\
4                    & 28              & 34.55        & 13.46        & 37.50          & 13.46           & 38.55        & 8.70         \\
8                    & 22              & 44.47        & 8.70         & 42.78          & 4.35            & 46.89        & 9.09         \\
16                   & 46              & 52.06        & 6.25         & 54.70          & 4.17            & 54.34        & 4.44         \\
32                   & 62              & 50.61        & 6.76         & 50.62          & 6.76            & 47.55        & 16.86        \\
64                   & 82              & 58.07        & 3.98         & 55.63          & 10.23           & 51.38        & 18.28        \\
128                  & 139             & 60.38        & 6.00         & 58.82          & 6.83            & 57.73        & 10.81        \\
256                  & 165             & 60.20        & 8.20         & 62.26          & 5.46            & 54.88        & 14.66        \\
512                  & 183             & 69.25        & 6.22         & 67.25          & 6.78            & 60.46        & 14.15        \\
999                  & 244             & 68.51        & 5.62         & 67.52          & 6.78            & 63.71        & 12.48        \\
1999                 & 295             & 69.36        & 6.40         & 68.61          & 7.07            & 64.88        & 10.38        \\
3999                 & 380             & 74.44        & 4.83         & 74.46          & 5.92            & 70.78        & 10.13        \\
7999                 & 425             & 80.34        & 3.56         & 79.01          & 4.30            & 75.14        & 8.80         \\
15999                & 554             & 80.65        & 4.91         & 79.33          & 5.34            & 73.27        & 9.80         \\
31999                & 609             & 80.17        & 4.88         & 79.73          & 5.18            & 75.35        & 11.98        \\
63999                & 680             & 81.73        & 3.97         & 80.41          & 5.12            & 75.13        & 10.66        \\
64000+               & 2658            & 81.93        & 4.59         & 80.13          & 6.04            & 73.95        & 12.09        \\ \cdashline{1-8}\noalign{\vskip 0.5ex}
Average                  & 352             & 61.58        & 5.72         & 61.57          & 6.29            & 58.46        & 10.82    \\ \bottomrule
\end{tabular}
\caption{Precision of translation and delete rates concerning source word types with varying frequencies. ``Freq. Bin'' and ``Counts'' indicate the frequency upper bounds and the count of each source type word. ``ACC'' and ``Delete'' indicate the precision and deletion rates of word prediction. LLM-SFT-S0.1 refers to conducting inference at a temperature setting of $0.1$.}
\label{tab:apprareword}
\end{table*}

==> tablesandfigures/c3_rarewords.tex <==
% \begin{table}[ht]
% \begin{tabular}{lcccc}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{Freq.(\textless{}=)}} & \multicolumn{2}{c}{NMT} & \multicolumn{2}{c}{LLM-SFT} \\ \cmidrule(r){2-5}
% \multicolumn{1}{c}{}                                       & ACC       & delete      & ACC        & delete      \\ \midrule
% 0                                                          & 0.61      & 0.10        & 0.66       & 0.07        \\
% 1                                                          & 0.48      & 0.20        & 0.65       & 0.00        \\
% 2                                                          & 0.44      & 0.04        & 0.37       & 0.09        \\
% 4                                                          & 0.62      & 0.08        & 0.59       & 0.09        \\
% 16                                                         & 0.61      & 0.16        & 0.66       & 0.07        \\
% 32                                                         & 0.62      & 0.16        & 0.68       & 0.09        \\
% 64                                                         & 0.71      & 0.11        & 0.68       & 0.12        \\
% 128                                                        & 0.71      & 0.14        & 0.73       & 0.08        \\
% 256                                                        & 0.73      & 0.14        & 0.73       & 0.10        \\
% 512                                                        & 0.75      & 0.12        & 0.76       & 0.11        \\
% 999                                                        & 0.78      & 0.10        & 0.72       & 0.15        \\
% 1999                                                       & 0.80      & 0.10        & 0.79       & 0.11        \\
% 3999                                                       & 0.83      & 0.09        & 0.78       & 0.12        \\
% 7999                                                       & 0.81      & 0.10        & 0.75       & 0.14        \\
% 15999                                                      & 0.79      & 0.12        & 0.78       & 0.14        \\
% 31999                                                      & 0.81      & 0.11        & 0.78       & 0.12        \\
% 64000                                                      & 0.79      & 0.12        & 0.78       & 0.14       \\ \bottomrule

% \end{tabular}
% \label{tab:rarewords}
% \caption{Word prediction accuracy and detect rate depended on word frequency.}
% \end{table}


% \begin{table}[ht]
% \begin{tabular}{lcccc}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{Freq.(\textless{}=)}} & \multicolumn{2}{c}{NMT} & \multicolumn{2}{c}{LLM-SFT} \\ \cmidrule(r){2-5}
% \multicolumn{1}{c}{}                                       & ACC       & delete      & ACC        & delete      \\ \midrule
% 0                                                          & 0.61      & 0.10        & 0.66       & 0.07        \\
% 1                                                          & 0.48      & 0.20        & 0.65       & 0.00        \\
% 2                                                          & 0.44      & 0.04        & 0.37       & 0.09        \\
% 4                                                          & 0.62      & 0.08        & 0.59       & 0.09        \\
% 16                                                         & 0.61      & 0.16        & 0.66       & 0.07        \\
% 32                                                         & 0.62      & 0.16        & 0.68       & 0.09        \\
% 64                                                         & 0.71      & 0.11        & 0.68       & 0.12        \\
% 128                                                        & 0.71      & 0.14        & 0.73       & 0.08        \\
% 256                                                        & 0.73      & 0.14        & 0.73       & 0.10        \\
% 512                                                        & 0.75      & 0.12        & 0.76       & 0.11        \\
% 999                                                        & 0.78      & 0.10        & 0.72       & 0.15        \\
% 1999                                                       & 0.80      & 0.10        & 0.79       & 0.11        \\
% 3999                                                       & 0.83      & 0.09        & 0.78       & 0.12        \\
% 7999                                                       & 0.81      & 0.10        & 0.75       & 0.14        \\
% 15999                                                      & 0.79      & 0.12        & 0.78       & 0.14        \\
% 31999                                                      & 0.81      & 0.11        & 0.78       & 0.12        \\
% 64000                                                      & 0.79      & 0.12        & 0.78       & 0.14       \\ \bottomrule

% \end{tabular}
% \label{tab:rarewords}
% \caption{Word prediction accuracy and detect rate depended on word frequency.}
% \end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{lllll}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{freq.(\textgreater{}=\#)}} & \multicolumn{2}{c}{NMT}       & \multicolumn{2}{c}{LLM-SFT}      \\ \cmidrule(r){2-5}
\multicolumn{1}{c}{}                                          & ACC           & delete        & ACC           & delete        \\ \midrule
0                                                             & 0.55          & 0.27          & \textbf{0.56} & \textbf{0.26} \\
1                                                             & 0.48          & 0.38          & \textbf{0.59} & \textbf{0.23} \\
2                                                             & \textbf{0.40} & \textbf{0.46} & 0.38          & 0.46          \\
4                                                             & \textbf{0.56} & \textbf{0.25} & 0.48          & 0.30          \\
16                                                            & 0.51          & 0.33          & \textbf{0.53} & \textbf{0.31} \\
32                                                            & 0.56          & 0.28          & \textbf{0.59} & \textbf{0.16} \\
64                                                            & 0.58          & 0.20          & \textbf{0.60} & \textbf{0.12} \\
128                                                           & \textbf{0.58} & 0.22          & 0.57          & \textbf{0.18} \\
256                                                           & 0.58          & 0.15          & \textbf{0.62} & \textbf{0.10} \\
512                                                           & 0.57          & 0.16          & \textbf{0.64} & \textbf{0.09} \\
999                                                           & 0.61          & 0.13          & \textbf{0.66} & \textbf{0.09} \\
1999                                                          & 0.61          & 0.11          & \textbf{0.68} & \textbf{0.06} \\
3999                                                          & 0.62          & 0.11          & \textbf{0.65} & \textbf{0.06} \\
7999                                                          & 0.58          & 0.12          & \textbf{0.64} & \textbf{0.07} \\
15999                                                         & 0.59          & 0.13          & \textbf{0.65} & \textbf{0.06} \\
31999                                                         & 0.60          & 0.12          & \textbf{0.66} & \textbf{0.06} \\
64000                                                         & 0.62          & 0.14          & \textbf{0.69} & \textbf{0.07} \\ \bottomrule
\end{tabular}
\label{tab:rarewords}
\caption{Word prediction accuracy and detect rate depended on word frequency.}
\end{table}

==> tablesandfigures/c4_sentlevel_comet.tex <==
\pgfplotsset{superb legend/.style={legend style                                = {draw=none,
                 legend columns                          = 3,
                 /tikz/every even column/.append style   = {column sep=0.5cm,
                 text width=7em},
                 /tikz/every odd column/.append style    = {column sep=0.15cm,
                  text width=7em},
                 }}}

\begin{figure}[ht]

    \centering
    % \includegraphics{}
  
\begin{tikzpicture}
\pgfplotsset{
every axis legend/.append style={at={(0.5,1.03)},anchor=south},
% every axis y label/.append style={at={(0.07,0.5)}}
}

\begin{axis}[
    legend columns=3,legend style={font=\small},
    % title={Data amount dependence of De-En translation quality},
    xlabel={\bf Sample Length},
    ylabel={\bf COMET-DA},
    xmin=-0.3, xmax=9.3,
    ymin=75, ymax=90,
    ytick={75,80,85,90},
    xtick={0,1,2,3,4,5,6,7,8,9},
    xticklabels={0,10,20,30,40,50,60,70,80,90},
    % x tick label style={rotate=45,anchor=east},
    % legend pos=north west,
    % legend pos=south east,
    % legend pos=outer north east,
    ymajorgrids=true,
    grid style=dashed,
    height=2.3in,
    width=0.48\textwidth,
    nodes near coords
]


\addplot[
    color=red,
    mark=triangle,
    mark options={scale=1.5}
    ]
    coordinates {
    (0.5,87.7)(1.5,85.6)(2.5,84.1)(3.5,82.9)(4.5,83.4)(5.5,83.6)(6.5,82.8)(7.5,81.7)(8.5,81.0)
    };
    \addlegendentry{LLM-SFT}

\addplot[
    color=blue,
    mark=square,
    nodes near coords style={yshift=-15pt},
    point meta=explicit symbolic
    ]
    coordinates {
    (0.5,87.2)[87.2](1.5,84.7)[84.7](2.5,83.3)[83.3](3.5,81.7)[81.7](4.5,81.6)[81.6](5.5,82.4)[82.4](6.5,81.2)[81.2](7.5,80.3)[80.3](8.5,78.9)[78.9]
    }; \addlegendentry{Enc2Dec}

\end{axis}



\end{tikzpicture}

% \caption{BLEU scores with different sample lengths for German-to-English MT systems. The length of less than $90$ words is sentence-level translation, otherwise is document-level translation. LLMs improve the long sentence translation performance and also continually perform good in document-level translation.}
\caption{COMET-DA scores for sentence-level translation of German-to-English MT systems with varying sample lengths.}
\label{fig:c3-sentlen-comet}

\end{figure}

% BLEU scores for German-to-English MT systems across varying sample lengths. Lengths of less than $90$ words correspond to sentence-level translation, while those exceeding this threshold pertain to document-level translation. LLMs enhance the performance of long sentence translation and consistently exhibit strong performance in document-level translation tasks.

==> tablesandfigures/c5_alignment_example.tex <==
\begin{table*}[ht]
% \begin{tabular}{lcccccccccccccccc}
\centering
\scalebox{0.65}{
\begin{tabular}{lllllllllllllllll}
\toprule
layer & 1      & 2  & 3      & 4      & 5      & 6  & 7      & 8    & 9      & 10     & 11     & 12    & 13    & 14     & 15    & 16     \\ \midrule
He    & T      & od & T      & .      & ,      & '  & ay     & '    & ,  & $\_$the   & .      & $\_$park & T     & T      & T     & T      \\
ute   & ay     & ay & '      & T      & od     & T  & T      & m    & T      & $\_$park  & od     & .     & od    & ,      & $\_$park & T      \\
$\_$ge   & ay     & $\_$I & $\_$park  & od     & .      & '  & T      & m    & T      & $\_$park  & $\_$going & .     & T     & od     & od    & od     \\
he    & ay     & ay & '      & ,      & '      & '  & od     & $\_$to  & T      & $\_$the   & od     & .     & od    & ,      & $\_$park & T      \\
$\_$ich  & T      & od & od     & ,      & $\_$the   & '  & od     & T    & T      & $\_$the   & .      & m     & $\_$park & T      & ,     & T      \\
$\_$in   & $\_$going & ,  & $\_$park  & T      & $\_$to    & T  & $\_$going & $\_$the & T      & $\_$going & ay     & .     & T     & $\_$park  & '     & $\_$I     \\
$\_$den  & T      & $\_$I & $\_$park  & T      & $\_$park  & '  & '      & od   & T      & $\_$the   & $\_$going & .     & T     & m      & '     & '      \\
$\_$Park & T      & ay & T      & T      & .      & '  & od     & ay   & $\_$I     & $\_$the   & T      & $\_$park & od    & T      & T     & T      \\
.     & ,      & ,  & $\_$going & T      & T      & ,  & $\_$park  & .    & '      & .      & T      & T     & '     & $\_$park  & $\_$the  & T      \\ \midrule \midrule
layer & 17     & 18 & 19     & 20     & 21     & 22 & 23     & 24   & 25     & 26     & 27     & 28    & 29    & 30     & 31    & 32     \\ \midrule
He    & od     & .  & od     & $\_$the   & $\_$going & ,  & .      & '    & $\_$I     & T      & od     & $\_$the  & od    & $\_$going & .     & $\_$park  \\
ute   & ,      & .  & T      & .      & $\_$going & ,  & $\_$park  & $\_$I   & '      & T      & '      & od    & od    & T      & ,     & '      \\
$\_$ge   & ,      & .  & od     & T      & $\_$going & ,  & .      & '    & m      & T      & od     & $\_$the  & od    & od     & '     & m      \\
he    & ,      & .  & T      & $\_$the   & $\_$going & ,  & T      & m    & $\_$going & T      & T      & T     & od    & T      & m     & $\_$going \\
$\_$ich  & '      & .  & T      & .      & $\_$going & ,  & .      & T    & T      & T      & '      & $\_$the  & od    & $\_$park  & $\_$to   & $\_$going \\
$\_$in   & .      & '  & ,      & ay     & T      & .  & od     & ,    & T      & T      & T      & T     & ay    & ,      & '     & '      \\
$\_$den  & .      & od & $\_$going & $\_$I     & od     & .  & ay     & '    & $\_$the   & T      & T      & $\_$the  & m     & ,      & '     & ay     \\
$\_$Park & $\_$the   & .  & T      & T      & T      & ,  & .      & $\_$I   & ,      & T      & '      & T     & od    & $\_$park  & .     & $\_$park  \\
.     & ,      & od & .      & $\_$going & $\_$park  & .  & .      & .    & ,      & T      & od     & ay    & .     & ,      & '     & '     \\ \bottomrule
\end{tabular}}
\caption{Word alignment with $32$ layers induced by the maximum attention score in LLM self-attention matrics. The left row is a German sentence ``Heute gehe ich in den Park.'', and its target English sentence is ``Today, I'm going to the park.''. Both sentences are tokenized by the LLama2 tokenizer.}
\label{tab:alignmentexample}
\end{table*}

==> tablesandfigures/c6_beam_search.tex <==

\pgfplotsset{superb legend/.style={legend style                                = {draw=none,
                 legend columns                          = 3,
                 /tikz/every even column/.append style   = {column sep=0.5cm,
                 text width=7em},
                 /tikz/every odd column/.append style    = {column sep=0.15cm,
                  text width=7em},
                 }}}

\begin{figure}
    \centering
    % \includegraphics{}
  
\begin{tikzpicture}
\pgfplotsset{
every axis legend/.append style={at={(0.5,1.03)},anchor=south},
% every axis y label/.append style={at={(0.07,0.5)}}
}
\begin{axis}[
    legend columns=3,legend style={font=\tiny},
    % title={Data amount dependence of De-En translation quality},
    xlabel={Data amount},
    ylabel={BLEU score},
    xmin=0, xmax=5,
    ymin=2, ymax=50,
    ytick={5,10,15,20,25,30,35,40,45},
    xticklabels={1,2,4,12},
    xtick={1,2,3,4},
    % x tick label style={rotate=45,anchor=east},
    % legend pos=north west,
    % legend pos=south east,
    % legend pos=outer north east,
    ymajorgrids=true,
    grid style=dashed,
    height=2.3in,
    width=0.5\textwidth,
    nodes near coords
]


\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (1,39.4)(2,40.7)(3,41.2)(4,41.7)
    };
    \addlegendentry{LLMs-SFT}



\end{axis}
\end{tikzpicture}

\caption{BLEU scores for German-to-English systems trained on $10k$ to $10M$ translation pairs.}
\label{fig:enter-label}

\end{figure}

==> tablesandfigures/c8_evaluation.tex <==
\subsection{Evaluation Issues}

We analyze three representative systems on WMT2023 {\em Discourse-Level Literary Translation} Chinese-English Testset. \textit{Commercial Translation System}: we use Google Translate,\footnote{\url{https://translate.google.com}.}, which usually performs state-of-the-art in translation performance. \textit{Commercial LLM Systems}: we employ GPT-4 (8K) API\footnote{\url{https://platform.openai.com}.} to translate documents, which is known for its extensive context modeling capabilities \cite{ouyangtraining-instructGPT,wang2023document}. \textit{Open-sourced LLM Models}: we enhance Llama-7b (2K)~\cite{touvron2023llama} on document-level translation by using the 200K general-domain document-level training set \cite{du2023on}.\footnote{All were conducted between August 1st and 30th, 2023.}

We use both automatic and human evaluation methods to evaluate above systems. About automatic evaluation, we employ document-level sacreBLEU (d-BLEU) as our metric, which is computed by matching n-grams in the whole document~\cite{liu2020multilingual,post2018call}. In terms of human evaluation, we propose a well-defined criterion by adapting multidimensional quality metrics (MQM) \cite{lommel2014multidimensional,wang2023findings} to fit the context of literary translation.\footnote{All evaluations are case-sensitive.}
According to the result in Table~\ref{tab:auto-vs-human}, we have:

\begin{itemize}[leftmargin=*,topsep=0.1em,itemsep=0.1em,parsep=0.1em]

\item \textbf{A certain degree of divergence is observed between human and automatic assessments.}
We computed a Pearson correlation coefficient of -0.53. This value, a moderate negative correlation coefficient of -0.53, indicates an inverse relationship between human and automatic evaluations. There is a certain degree of discrepancy between human and automatic evaluation, which potentially provides complementary reference points when measuring the quality of document-level translations. This finding underscores the importance of integrating both human and automatic evaluation methods in assessing machine translation systems. It also highlights potential limitations in current automatic evaluation approaches when gauging the quality of machine translations.

human-like / human-preferenced

\end{itemize}


\begin{table}[t]
    \centering
    \begin{tabular}{c r r}
     \toprule
     {\bf System} & {\color{red} \bf MQM} & {\color{blue}\bf d-BLEU}\\
    \midrule
   GPT-4 & \cellcolor{red!30} 54.81 & \cellcolor{blue!15} 43.7\\
   Llama-MT & \cellcolor{red!15} 28.40  & \cellcolor{blue!5} 43.1\\
   Google & \cellcolor{red!5} 22.66  & \cellcolor{blue!30} 47.3\\
    \bottomrule
    \end{tabular}
    \caption{The comparison between human (MQM) vs. automatic (d-BLEU) evaluation methods over three representative systems, with a color scale to denote the evaluation ranking. The Pearson correlation coefficient between MQM and d-BLEU is $-0.53$.}
    % \caption{The comparison between human (MQM) vs. automatic (d-BLEU) evaluation methods over three representive systems. The results are presented using a color scale to denote the ranking of each system based on these evaluations.}
    \label{tab:auto-vs-human}
\end{table}

==> tablesandfigures/dataformat_simple.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{cp{6cm}} 
    \toprule
        \bf Type & \multicolumn{1}{l}{\bf Data Format} \\ \midrule
          \bf SFT   & Below is an instruction that ... \\ \cdashline{2-2}\noalign{\vskip 0.5ex}
             & \#\#\# Instruction: Translate the follow ... \\ \cdashline{2-2}\noalign{\vskip 0.5ex}
             & \#\#\# Input: Haben Sie einen Blick ... \\ \cdashline{2-2}\noalign{\vskip 0.5ex}
             & \#\#\# Response: Have you looked at ... \\ \midrule

        \bf CPT & [German]: Haben Sie einen Blick ... [English]: Have you looked at other ... \\ \bottomrule
            
    \end{tabular}
    \caption{An illustration of two data formats utilized for training LLMs, where SFT represents supervised finetuning, and CPT denotes continual pertaining.}
    \label{tab:insdata}
\end{table}


% \begin{table}[h]
%     \centering
%     \begin{tabular}{cp{6cm}} 
%     \toprule
%         \bf Type & \multicolumn{1}{l}{\bf Data Format} \\ \midrule
%           \bf SFT   & Below is an instruction that describes a task, paired with an input that provides further context. Write a response that appropriately completes the request. \\ \cdashline{2-2}\noalign{\vskip 0.5ex}
%              & \#\#\# Instruction: Translate the following sentences from German to English. \\ \cdashline{2-2}\noalign{\vskip 0.5ex}
%              & \#\#\# Input: Haben Sie einen Blick auf andere Restaurants in der Nähe mit ähnlicher Küche geworfen? \\ \cdashline{2-2}\noalign{\vskip 0.5ex}
%              & \#\#\# Response: Have you looked at other nearby restaurants with similar cuisine? \\ \midrule

%         \bf CPT & [German]: Haben Sie einen Blick auf andere Restaurants in der Nähe mit ähnlicher Küche geworfen? [English]: Have you looked at other nearby restaurants with similar cuisine? \\ \bottomrule
            
%     \end{tabular}
%     \caption{An illustration of two data formats utilized for training LLMs, where SFT represents supervised finetuning, and CPT denotes continual pertaining.}
%     \label{tab:insdata}
% \end{table}
